Learning Transformations To Reduce the Geometric Shift in Object Detection

The performance of modern object detectors drops when the test distribution differs from the training one. Most of the methods that address this focus on object appearance changes caused by, e.g., different illumination conditions, or gaps between synthetic and real images. Here, by contrast, we tackle geometric shifts emerging from variations in the image capture process, or due to the constraints of the environment causing differences in the apparent geometry of the content itself. We introduce a self-training approach that learns a set of geometric transformations to minimize these shifts without leveraging any labeled data in the new domain, nor any information about the cameras. We evaluate our method on two different shifts, i.e., a camera's field of view (FoV) change and a viewpoint change. Our results evidence that learning geometric transformations helps detectors to perform better in the target domains.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system("latexmk -cd -pdf \"$_[0]\" " );
    }
}

==> tables/supp_da.tex <==
\begin{table}[h]


  \centering
  \begin{tabular}{lcc}
    \toprule

    Method     & Car AP@0.5 & Pedestrian AP@0.5 \\
    \midrule
    ~\cite{li2022cross} & 77.2 & 63.5\\
    Ours(N=9) & 80.4\tiny{$\pm$0.15} & Ours(N=5) 65.3\tiny{$\pm$ 0.37}\\
    \bottomrule
  \end{tabular}
    \caption{FoV Adaptation }
      \label{tab:supp_da}
\end{table}

==> tables/supp_tau_lamda.tex <==
% !TEX root = ../supp.tex
% !TEX spellcheck = en-US
\begin{table}[h]
  \caption{Mean Teacher Training }
  \label{tab:supp_tau_lamda}
  \centering
  \begin{tabular}{lc}
    \toprule

    Kind     & Details  \\
    \midrule
    Random Crop & Relative Range: $[0.3 ,1]$ \\

    Color Jitter & Brightness=$.5$, Hue=$.3$\\
    \bottomrule
  \end{tabular}
\end{table}

==> tex/limit_societal_impact.tex <==
\section{Broader impact}
\label{sec:broader_impact}
With the growing number of applications of object detection, it is important to understand the biases induced by the training dataset. While domain adaptation methods can alleviate such biases, existing works has focused on object appearance variations. Here, we study a different type of bias, namely, geometric ones. As such, and as demonstrated by our experiments, our approach can help object detectors to generalize better to train-test condition changes. While this could facilitate deployment in real-world applications, our approach does not offer robustness guarantees, particularly to adversarial attacks. As such, it can potentially be diverted to yield dangerous situations in applications such as autonomous navigation.


%and our method is a step in this direction. We reduce the geometric shifts occuring between the training and test data, which helps in better generalization of the object detectors.  }
